A Framework for Modelling, Verification and Transformation of Concurrent Imperative Programs

The paper gives a detailed presentation of a framework, embedded into the simply typed higher-order logic and aimed at the support of sound and structured reasoning about various properties of models of imperative programs with interleaved computations. As a case study, a model of the Peterson's mutual exclusion algorithm will be scrutinised in the course of the paper illustrating applicability of the framework.

==> sedindex <==
#! /bin/sh
#
#sedindex - shell script to create indexes, preprocessing LaTeX's .idx file
#
#  puts strings prefixed by * into \tt font
#    terminator characters for strings are |!@{}
#
# a space terminates the \tt part to allow \index{*NE theorem}, etc.
#
# change *"X"Y"Z"W  to  "X"Y"Z"W@{\tt "X"Y"Z"W}
# change *"X"Y"Z    to  "X"Y"Z@{\tt "X"Y"Z}
# change *"X"Y      to  "X"Y@{\tt "X"Y}
# change *"X        to  "X@{\tt "X}
# change *IDENT  to  IDENT@{\tt IDENT}  
#    where IDENT is any string not containing | ! or @
# FOUR backslashes: to escape the shell AND sed
sed -e "s~\*\(\".\".\".\".\)~\1@{\\\\tt \1}~g
s~\*\(\".\".\".\)~\1@{\\\\tt \1}~g
s~\*\(\".\".\)~\1@{\\\\tt \1}~g
s~\*\(\".\)~\1@{\\\\tt \1}~g
s~\*\([^ |!@{}][^ |!@{}]*\)~\1@{\\\\tt \1}~g" $1.idx | makeindex -c -q -o $1.ind

